A New Term Rewriting Characterisation of ETIME functions

Adopting former term rewriting characterisations of polytime and exponential-time computable functions, we introduce a new reduction order, the Path Order for ETIME (POE* for short), that is sound and complete for ETIME computable functions. The proposed reduction order for ETIME makes contrasts to those related complexity classes clear.

==> conclusion.tex <==
\section{Conclusion}\label{s:conclusion}

\begin{figure}%[t]
\centering
\begin{tabular}{c|c|c|c}
\hline 
Complexity classes \ & \ Recursion schemata \ & 
\multicolumn{2}{c}{Comparison in reduction orders} \\
\hline
& & \ normal arguments \ & \ safe arguments \ \\
\hline
Polytime & \textbf{SRN} & 
product & product \\
ETIME & $\oneSNRN$ & product & full comparison \\
EXP & \textbf{SNRN} & full comparison & full comparison \\
\hline
\end{tabular} 
%
\caption{Contrast to related characterisations}
\label{fig:conclusion}
\end{figure}

